An Implementation of the Optimal Scheme for Energy Efficient Bus Encoding

In computer system buses, most of the energy is spent to change the voltage of each line from high to low or vice versa. Bus encoding schemes aim to improve energy efficiency by limiting the number of transitions between successive uses of the bus. We propose an implementation of the optimal code with reduced number of clock cycles.

==> StableFigures/tabComplexity.tex <==
\begin{table}[t]
    \centering
    \caption{{Complexity analysis summary in terms of elementary operations.}}
    %Asymptotic thresholds analysis varying the number of antennas $M$. The analysis is conducted adopting $\Lambda^{\prime}(1) = 3.0$, the corresponding optimal distribution $\Lambda(x) = x^3$, $N_\mathrm{P} = 64$, $t = 10$, $N_\mathrm{D} = 256$.}
    \label{tab:complexity}
    \small
    {
    \begin{tabular}{cl}
        \toprule
        \rowcolor[gray]{.95}
        \textbf{Scheme} & \multicolumn{1}{c}{$\mathcal{C}_\mathrm{enc}$}\\
        \midrule
        DBI   & $2 \times \left[ \mathcal{C}_\mathrm{w}(n) + \mathcal{C}_\mathrm{c}(\lceil \log_2 n \rceil) \right]$ \\
        PI  & $2b \times \left[ \mathcal{C}_\mathrm{w}(k/b) + \mathcal{C}_\mathrm{c}(\lceil \log_2 k/b \rceil) \right]$ \\
        %\rowcolor[gray]{.95}
        PR/RI  & $2^b \times \left[ \mathcal{C}_\mathrm{w}(n) + \mathcal{C}_\mathrm{c}(\lceil \log_2 n \rceil) \right]$ \\
        SI  & $\min\{k,2^b\} \times \left[ \mathcal{C}_\mathrm{w}(n) + \mathcal{C}_\mathrm{c}(\lceil \log_2 n \rceil) \right]$ \\
        %\rowcolor[gray]{.95}
        Gen. Opt. & $\left[(n + 2) D_\mathrm{opt}(k,b)+d_\mathrm{max} + 1\right] \times \mathcal{C}_\mathrm{c}(n)$ \\
        \bottomrule
    \end{tabular}
    }
\end{table}


==> StableFigures/tableSummary.tex <==
\begin{table}[t]
    \centering
    \caption{{{Examples for some choices of the system parameters}}}
    \label{tab:summary}
    \small
    {
    \begin{tabular}{ccccccc}
        \toprule
        \rowcolor[gray]{.95}
        \textbf{Scheme} & $k$ & $D_\mathrm{unc}(k)$ & $b$ & $k/n$ & $ D(k,b)$ & $\eta$ [$\%$]\\
        \midrule
        \multirow{2}[2]{*}{DBI} & $8$ & $4$ & $1$ & $0.889$ & $3.27$ & $18.3$\\
        \cmidrule{2-7}
        & $64$ & $32$ & $1$ & $0.985$ & $29.27$ & $8.5$\\
        \midrule
        \multirow{4}[5]{*}{PI} & \multirow{2}[2]{*}{$8$} & \multirow{2}[2]{*}{$4$} & $2$ & $0.800$ & $3.12$ & $21.9$ \\
        \cmidrule{4-7}
        & & & $4$ & $0.667$ & $3.00$ & $25.0$\\
        \cmidrule{2-7}
        & \multirow{2}[2]{*}{$64$} & \multirow{2}[2]{*}{$32$} & $4$ & $0.941$ & $27.32$ & $14.6$\\
        \cmidrule{4-7}
        & & & $8$ & $0.889$ & $26.16$ & $18.3$\\
        \midrule
        \multirow{4}[5]{*}{RI} & \multirow{2}[2]{*}{$8$} & \multirow{2}[2]{*}{$4$} & $2$ & $0.800$  & $3.14$ & $21.4$ \\
        \cmidrule{4-7}
        & & & $4$ & $0.667$ & $2.91$ & $27.4$\\
        \cmidrule{2-7}
        & \multirow{2}[2]{*}{$64$} & \multirow{2}[2]{*}{$32$} & $4$ & $0.941$ & $26.64$ & $16.7$\\
        \cmidrule{4-7}
        & & & $8$ & $0.889$ & $24.10$ & $24.7$ \\
        \midrule
        \multirow{4}[5]{*}{Opt.} & \multirow{2}[2]{*}{$8$} & \multirow{2}[2]{*}{$4$} & $2$ & $0.800$  & $3.04$ & $23.8$ \\
        \cmidrule{4-7}
        & & & $4$ & $0.667$ & $2.64$ & $34.1$\\
        \cmidrule{2-7}
        & \multirow{2}[2]{*}{$64$} & \multirow{2}[2]{*}{$32$} & $4$ & $0.941$ & $25.92$ & $19.0$\\
        \cmidrule{4-7}
        & & & $8$ & $0.889$ & $23.54$ & $26.4$ \\
        \bottomrule
    \end{tabular}
    }
\end{table}


==> StableFigures/tableSummary2.tex <==
\begin{table}[t]
    \centering
    \caption{Examples for some choices of the system parameters}
    \label{tab:summary}
    \small
    {
    \begin{tabular}{ccccccc}
        \toprule
        \rowcolor[gray]{.95}
        \textbf{Scheme} & $k$ & $D_\mathrm{unc}(k)$ & $b$ & $k/n$ & $ D(k,b)$ & $\eta$ [$\%$]\\
        \midrule
        \multirow{2}{*}{DBI} & $8$ & $4$ & $1$ & $0.889$ & $3.27$ & $18.3$\\
        \cmidrule{2-7}
         & $64$ & $32$ & $1$ & $0.985$ & $29.27$ & $8.5$\\
        \midrule
        \multirow{3}{*}{PI} & $8$ & $4$ & $2$ & $0.800$ & $3.12$ & $21.9$ \\
        \cmidrule{2-7}
        & \multirow{2}{*}{$64$} & \multirow{2}{*}{$32$} & $4$ & $0.941$ & $27.32$ & $14.6$\\
        \cmidrule{4-7}
        & & & $8$ & $0.889$ & $26.16$ & $18.3$\\
        \midrule
        \multirow{3}{*}{RI} & $8$ & $4$ & $2$ & $0.800$  & $3.14$ & $21.4$ \\
        \cmidrule{2-7}
        & \multirow{2}{*}{$64$} & \multirow{2}{*}{$32$} & $4$ & $0.941$ & $26.64$ & $16.7$\\
        \cmidrule{4-7}
        & & & $8$ & $0.889$ & $24.10$ & $24.7$ \\
        \midrule
        \multirow{3}{*}{Opt.} & $8$ & $4$ & $2$ & $0.800$  & $3.04$ & $23.8$ \\
        \cmidrule{2-7}
        & \multirow{2}{*}{$64$} & \multirow{2}{*}{$32$} & $4$ & $0.941$ & $25.92$ & $19.0$\\
        \cmidrule{4-7}
        & & & $8$ & $0.889$ & $23.54$ & $26.4$ \\
        \bottomrule
    \end{tabular}
    }
\end{table}

